Does Data Augmentation Lead to Positive Margin?

Data augmentation (DA) is commonly used during model training, as it significantly improves test error and model robustness. DA artificially expands the training set by applying random noise, rotations, crops, or even adversarial perturbations to the input data. Although DA is widely used, its capacity to provably improve robustness is not fully understood. In this work, we analyze the robustness that DA begets by quantifying the margin that DA enforces on empirical risk minimizers. We first focus on linear separators, and then a class of nonlinear models whose labeling is constant within small convex hulls of data points. We present lower bounds on the number of augmented data points required for non-zero margin, and show that commonly used DA techniques may only introduce significant margin after adding exponentially many points to the data set.

==> upper_bound_inradius_camera.tex <==
   % \subsection{Upper Bounds on Margin}

   \paragraph{Upper bounds on margin.} Finally, we show that for certain $S$, the margin bounds in Theorems \ref{thm:nonlinear1} and \ref{thm:nonlinear2} are tight up to constants. Suppose $S = \{(x_1,1),(x_2,-1)\}$, and $S'$ is generated by Algorithm \ref{alg:data_aug}. We have the following result:
   
    \begin{theorem}\label{thm:nonlinear3}
        Fix $\epsilon \in [0,\infty]$ and $r > 0$. There are absolute constants $C_1, C_2$ such that if $N> d$ and $\mR_\epsilon(S^{\aug}) \neq \emptyset$, then with probability at least $1 - 2e^{-C_2 d \log(N/d)}$, $\exists f \in \mR_\epsilon(S^{\aug})$ such that
        \begin{equation}\label{eq:upper_circumradius}
        \gamma_f(S,S') \leq \sqrt{C_1\dfrac{\log(2N/d)}{d}}r.
        \end{equation}
    \end{theorem}

   This theorem can be extended to settings where $S_+$ and $S_-$ are not singletons. Suppose we can decompose $S_+$ and $S_-$ into clusters $\{S_{+,1},\ldots, S_{+,k}\}$ and $\{S_{-,1},\ldots, S_{-,l}\}$ such that each cluster has size at most $m$, $R(S_{+,i}), R(S_{-,j}) = O(\sqrt{\log(N/d)/d}r)$, and the distance between any two clusters is $\Omega(\epsilon)$. One can show that if we apply Algorithm \ref{alg:data_aug}, then with high probability, we can find $f \in \mR_\epsilon(S^{\aug})$ satisfying a version of inequality~\eqref{eq:upper_circumradius}, where $N$ is replaced by $mN$. If $m = O(1)$, then we find that Theorems \ref{thm:nonlinear1} and \ref{thm:nonlinear2} are tight up to constants.
